Modeling Hybrid Systems in the Concurrent Constraint Paradigm

Hybrid systems, which combine discrete and continuous dynamics, require quality modeling languages to be either described or analyzed. The Concurrent Constraint paradigm (ccp) is an expressive declarative paradigm, characterized by the use of a common constraint store to communicate and synchronize concurrent agents. In this paradigm, the information is stated in the form of constraints, in contrast to the variable/value style typical of imperative languages. Several extensions of ccp have been proposed in order to model reactive systems. One of these extensions is the Timed Concurrent Constraint Language (tccp) that adds to ccp a notion of discrete time and new features to model time-out and preemption actions. The goal of this paper is to explore the expressive power of tccp to describe hybrid systems. We introduce the language Hy-tccp as a conservative extension of tccp, by adding a notion of continuous time and new constructs to describe the continuous dynamics of hybrid systems. In this paper, we present the syntax and the operational semantics of Hy-tccp together with some examples that show the expressive power of our new language.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{S. Escobar (Ed.): XIV Jornadas sobre Programaci\'on\\ 
y Lenguajes, PROLE 2014, Revised Selected Papers\\
EPTCS 173, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.173.1}{10.4204/EPTCS.173.1}}

